Dangling-Aware Entity Alignment with Mixed High-Order Proximities

We study dangling-aware entity alignment in knowledge graphs (KGs), which is an underexplored but important problem. As different KGs are naturally constructed by different sets of entities, a KG commonly contains some dangling entities that cannot find counterparts in other KGs. Therefore, dangling-aware entity alignment is more realistic than the conventional entity alignment where prior studies simply ignore dangling entities. We propose a framework using mixed high-order proximities on dangling-aware entity alignment. Our framework utilizes both the local high-order proximity in a nearest neighbor subgraph and the global high-order proximity in an embedding space for both dangling detection and entity alignment. Extensive experiments with two evaluation settings shows that our framework more precisely detects dangling entities, and better aligns matchable entities. Further investigations demonstrate that our framework can mitigate the hubness problem on dangling-aware entity alignment.

==> intro.tex <==
\section{Introduction}

% == muhao == 
% 1. Background: what is the EA task and why this is an important problem;
% 2. Motivation and challenges: One emerging and practical challenge for EA is the problem of dangling entities. There are some preliminary attempts which make inference only based on first-order proximity: what is the common shortage of all existing solutions? How is this going to motivate a different solution in our research?
% 3. A new solution: what is the new principle? why is it practical?
% 4. In this paper ... 
% (5) the main contributions of this paper are 2/3/4-folds.
% =========

% the first paragraph: 1. the importance of KG (essential build blocks of many application); 2. Constructing costly and incompleteness. 3) To mitigate this, we have EA. 4) EA is a task to xxx (brief intro) 5) some representative works on EA and how they did it (embedding-based EA).
Knowledge graphs (KGs) have become an essential build block of many real-world applications \citep{ji2021survey}. 
In spite of the importance, many KGs are %incomplete and constructing them can be costly 
independently created without considering the
interchangeable and complementary nature of domain knowledge \citep{chen2020multilingual}. 
To mitigate this, entity alignment %combining information from multiple graphs aims 
seeks to identify equivalent entities in different KGs, therefore allowing complementary
knowledge to be automatically combined and migrated across individual KGs \cite{sun-etal-2020-knowledge}.
% , and provide more powerful knowledge representations for downstream applications. 
Specifically, entity alignment is a task to identify entities with the same real-world meaning from different KGs. For example, in multilingual KGs, English entity xxx and its Chinese counterpart entity xxx should be identified through entity alignment.
Recently, several embedding-based entity alignment methods have been proposed \citep{chen_MTransE, wang-etal-2018-cross-lingual, cao-etal-2019-multi, Fey2020Deep, sun-etal-2020-knowledge}. 
In general, embedding-based methods learn a embedding space where similar entities are placed closely and nearest neighbor search is conducted to retrieve entities that should be aligned. 
% In general, embedding-based methods jointly learn low-dimensional embeddings for different KGs and ensure that similar entities are placed closely in a latent space. After that, the nearest neighbor search is conducted to retrieve entities which should be aligned.  

% the second paragraph: 1. despite the effectiveness, previous methods neglect dangling entities. 2. To make the setting more realistic, Zequn ACL 21 proposes to consider dangling entities. briefly introduce the ways handling dangling entities. 3. However, they only consider first-order proximity (or individual-level proximity). The neighborhood information is important to identify the dangling entities. 
\muhao{Can directly start this paragraph by stating that, towards practical entity alignment, an emerging challenge is to resolve the dangling entity problem... (what is this problem? why is it practical in real-world scenarios? why challenging?)}
Despite the effectiveness of previous embedding-based methods, they cannot identify entities without counterpart alignment across KGs (named \textit{dangling entities}). 
The reason is that they generally assume any source entity can be aligned to a single counterpart in the target KG (i.e., one-to-one mapping from source KG to target KG), which is intrinsically unrealistic in real-world KGs. 
Under one-to-one mapping assumption, previous methods always predict a counterpart for a given source entity regardless whether it is a dangling entity, and may not be able to effectively align KGs in real-world scenarios.  

% (other transitions? Or maybe start a new paragraph) 
Recently, \citet{sun_no_match} redefine the entity alignment task with the consideration of dangling entities, which is more realistic. 
In this setting, conducting entity alignment consist of two parts: 1) given a source entity, determine whether a counterpart exists in the target KG (i.e., whether it is a matchable entity); 2) retrieve counterparts only for matchable entities. 
Consequently, a model aiming to perform well on this realistic setting also need to effectively generate valid predictions (i.e, matchable entities). 
Although some preliminary attempts \citep{sun_no_match} have been proposed to identify dangling entities, they have two major drawbacks. Firstly, they only consider the first-order proximity (namely, pairwise similarity) between source and target entities. 
Specially, they mainly encourage dangling entities to be isolated by enforcing a margin between a dangling entity and its nearest neighbor.
% jc: need to further explain why first-order proximity is not good enough?
We argue that \textit{high-order proximity} should be considered to better detect dangling entities and further facilitate entity alignment.  
For instance, intuitively, if a given source entity and its nearest target entity are mutually nearest, it is less likely to be a dangling entity.
% jc: this example is not clear to reflect high-order proximity? 
In this case, rather than only consider the proximity from source to target, the proximity through the reverse direction (i.e., from target to source) is also useful for detection dangling entities. 
The second shortcoming of previous attempts is that they neglect global information since they merely optimize entity-level loss for entity alignment without considering entity distributions. 
To explain, a desirable model can \textit{globally} align the distributions of matchable source and target entities instead of only aligning labeled entity pairs.
Furthermore, dangling entity distribution can be also considered to achieve some desirable relationships between it and other matchable entity distribution. 

% how to talk about the optimal transport and relate it a global solution. 
% the third paragraph: 
Motivated by the aforementioned drawbacks of previous work, in this study, we design a framework which can 1) utilize high-order proximity (e.g., source -> target -> source) for dangling entity detection and 2) obtain a global alignment by aligning two entity distributions while considering dangling entity distribution. 
The principle to utilize high-order proximity is that dangling entities should have different proximity distributions of their first-order and second-order neighborhoods compared with matchable entities. 
% The principle to align two distributions: ...
To exploit high-order proximity, the first component in our framework utilizes the similarity scores between a source entity and its neighbors (both first-order and second-order) for dangling detection.
Specifically, given a source entity $s$, using nearest neighbor search from source KG to target KG, we can get top $k$ nearest target entities and the first-order similarities between $k$ nearest target entities and the source entity $s$. 
Then through the reverse direction (from target KG to source KG), given the k target entities, the model retrieves some nearest source entities and calculates the second-order similarities (from the perspective of the source entity $s$). 
Using the first- and second-order similarities as an input, a multilayer perceptron (MLP) is trained to determine whether $s$ is a dangling entity. 

To obtain global information and consider entity distributions, the second main component is an entity alignment plugin based on Optimal Transport (OT). 
It aims to minimize the transportation cost of converting the distribution of matchable source entity embedding to that of matchable target entity embedding. 
At the same time, we design an additional loss to encourage a large distance between dangling entity distribution and matchable target entity distribution in order to better isolate dangling entities. 

The contributions of this work are three-fold: 




